Integral and Series Representations of Riemann's Zeta function, Dirichelet's Eta Function and a Medley of Related Results

Contour integral representations for Riemann's Zeta function and Dirichelet's Eta (alternating Zeta) function are presented and investigated. These representations flow naturally from methods developed in the 1800's, but somehow they do not appear in the standard reference summaries, textbooks or literature. Using these representations as a basis, alternate derivations of known series and integral representations for the Zeta and Eta function are obtained on a unified basis that differs from the textbook approach, and results are developed that appear to be new.

==> by_Parts.tex <==
By simple manipulation of the integral representations given, it is possible to obtain new series representations. Starting from the integral representation (\ref{ZetaC0}), integrate by parts, giving

\begin{equation}
\mapleinline{inert}{2d}{Zeta(s) =
sin(1/2*Pi*s)/(2^(1-s)-1)*Pi^2/(-1/2*s+1)*Int(t^(-s+2)*hypergeom([-1/2
*s+1],[3/2, 2-1/2*s],1/4*t^2*Pi^2)/sinh(Pi*t)^3*cosh(Pi*t),t = 0 ..
infinity);}{%
\maplemultiline{
\zeta (s)={\displaystyle \frac {\mathrm{sin}({\displaystyle 
\pi \,s/\,2} )\,\pi ^{2}}{(2^{(1 - s)} - 1)\,( - 
{\displaystyle s\,/2}  + 1)}}  \\
\times {\displaystyle \int _{0}^{\infty }} {\displaystyle \frac {t^{2- 
s}\,\mathrm{_{1}F_{2}}( - {\displaystyle \frac {s}{2}}  + 1
; \,{\displaystyle \frac {3}{2}} , \,2 - {\displaystyle \frac {
s}{2}} ; \,{\displaystyle \frac {t^{2}\,\pi ^{2}}{4}} )\,
\mathrm{cosh}(\pi \,t)}{\mathrm{sinh}^{3} (\pi \,t) }} \,dt \hspace*{3cm} \sigma<0 \,\, ,
} 
%
\label{Int1F2}
}
\end{equation}

where the hypergeometric function arises because of \cite{Luke}, Eq.6.2.11(6). Write the hypergeometric function as a (uniformly convergent) series, thereby permitting the sum and integral to be interchanged, apply a second integration by parts, and find

\begin{equation}
\mapleinline{inert}{2d}{Zeta(s) =
sin(1/2*Pi*s)*Pi*Sum(Pi^(2*k)/GAMMA(2*k+2)*Int(1/sinh(Pi*t)^2*t^(-s+1+
2*k),t = 0 .. infinity),k = 0 .. infinity)/(2^(1-s)-1);}{%
\[
\zeta (s)={\displaystyle \left( \frac {\pi}{2^{1 - s} - 1} \right )} \,{\displaystyle \mathrm{sin}({\displaystyle 
\pi \,s/2} )\, \! {\displaystyle \sum _{k=
0}^{\infty }} \, {\displaystyle \frac {\pi ^{2\,k}}{
\Gamma (2\,k + 2)}} \,{\displaystyle \int _{0}^{\infty }} 
{\displaystyle \frac {t^{1 - s  + 2\,k}}{\mathrm{sinh}^{2} (\pi \,
t) }} \,dt  } 
\hspace*{3cm} \sigma<0 \, \, .
\]
%
\label{SumInt}
}
\end{equation}

Identify the integral in (\ref{SumInt}) using (\ref{GR527.1}) giving
\begin{equation}\mapleinline{inert}{2d}{Zeta(s) =
sin(1/2*Pi*s)*2^s*Pi^(s-1)*Sum(2^(-2*k)*Zeta(-s+1+2*k)/GAMMA(2*k+2)*GA
MMA(-s+2+2*k),k = 0 .. infinity)/(2^(1-s)-1);}{%
\[
\zeta (s)={\displaystyle \frac {2^{s}\,\pi ^{s - 1}\, \mathrm{sin}({\displaystyle 
\pi\,s/2 } )\,}{2^{1 - s} - 1} \, 
{\displaystyle \sum _{k=0}^{\infty }} \,{\displaystyle \frac {2^{
- 2\,k}\,\zeta ( - s + 1 + 2\,k)\,\Gamma ( - s + 2 + 2\,k)}{
\Gamma (2\,k + 2)}}  }   
\]
%
\label{ZGamSum}
}
\end{equation}
valid for all values of $\sigma$ by the ratio test and the principle of analytic continuation. This result, which appears to be new, can be rewritten by extracting the $k=0$ term, and applying (\ref{functional}) to yield

\begin{equation}\mapleinline{inert}{2d}{Zeta(s) =
sin(1/2*Pi*s)*2^s*Pi^(s-1)*Sum(2^(-2*k)*Zeta(-s+1+2*k)/GAMMA(2*k+2)*GA
MMA(-s+2+2*k),k = 1 .. infinity)/(2^(1-s)-2+s);}{%
\[
\zeta (s)={\displaystyle \frac {2^{s}\,\pi ^{s - 1}\,\mathrm{sin}({\displaystyle \pi\,s/2 } )\,  \! 
} {2^{1 - s} - 2 + s}} {\displaystyle \sum _{k=1}^{\infty }} \,{\displaystyle \frac {2^{
- 2\,k}\,\zeta ( - s + 1 + 2\,k)\,\Gamma ( - s + 2 + 2\,k)}{
\Gamma (2\,k + 2)}}   
\],
%
\label{SumInt2}
}
\end{equation}


a representation, valid for all values of $s$, that is reminiscent of the following similar sum recently obtained by Tyagi and Holm (\cite{TyHo} Eq.(3.5))

\begin{equation}
\zeta (s) = \frac{\pi^{s-1}}{1-2^{1-s}} \mathrm{sin}( \pi\,s/2)\sum _{k=1} ^{\infty} \frac{(2-2^{s-2k})\,\zeta(-s+1+2k)\Gamma(-s+1+2k) }{\Gamma(2k+2)} \hspace*{2cm}  \sigma>{0}\,  \footnote{by Gauss' test}
\label{TyHo}
\end{equation}

Eq. (\ref{SumInt2}) can also be rewritten in the form
\begin{equation}
\zeta(s)=\frac{1}{\Gamma(s)(2^{s}-1-s)}\sum _{k=1} ^{\infty} \frac{2^{-2k} \zeta(s+2k)\Gamma(1+s+2k)}{\Gamma(2k+2)}
\label{SumInt2a}
\end{equation}
by replacing $s\rightarrow 1-s$ and applying (\ref{functional}).\newline

With reference to (\ref{ContInt}), express the numerator $\it{cosine}$ factor as a difference of exponentials each of which in turn is written as a convergent power series in $\pi\,(c+it)$, recognize that the resulting series can be interchanged with the integral and each term identified using (\ref{ContIntEta1}) to find 

\begin{equation}
\mapleinline{inert}{2d}{zeta(s) =
-Pi^(1/2)*Sum((-1/4*Pi^2)^k/GAMMA(k+1/2)/GAMMA(k+1)*eta(s-2*k),k = 0
.. infinity);}{%
\[
\zeta (s)= - \sqrt{\pi }\, \left(  \! {\displaystyle \, \sum _{k=0}
^{\infty }} \,{\displaystyle \frac {( - {\displaystyle {\pi
 ^{2}/4}} )^{k}\,\eta (s - 2\,k)}{\Gamma (k + {1/2} )\,\Gamma (k + 1)}}  \!  \right)\,.  \hspace*{2cm} \sigma >1 
\]
%
\label{Zsum1}
}
\end{equation}

A more interesting variation of (\ref{Zsum1}) can be obtained by applying (\ref{Eta=Zeta}) and explicitly identifying the $k=0$ term of the sum giving 

\begin{equation}
\mapleinline{inert}{2d}{zeta(s) =
-1/2*Pi^(1/2)*Sum((-1/4*Pi^2)^k/GAMMA(k+1/2)/GAMMA(k+1)*(1-2^(1-s+2*k)
)*Zeta(s-2*k),k = 1 .. infinity)/(1-2^(-s));}{%
\[
\zeta (s)= - {\displaystyle \frac {1}{2}} \,{\displaystyle 
\frac { \! {\displaystyle \sum _{k=1}^{
\infty }} \,{\displaystyle \frac {( - {\displaystyle {\pi 
^{2}}} )^{k}\,(1 - 2^{1 - s + 2\,k}) }{
\Gamma (2k + 1)}\zeta (s - 2\,k) }  \! 
 }{1 - 2^{- s}}}, 
\]
%
\label{Zsum1a}
}
\end{equation}

a convergent representation if $\sigma >1$ (by Gauss' test). An immediate consequence is the identification

\begin{equation}
\zeta(2) = - \frac {\pi^{2}} {3} \zeta(0) .
\end{equation}

because only the $k=1$ term in the sum contributes when $s=2$. Additionally, when $s=2n$, (\ref{Zsum1a}) terminates at $n$ terms, becoming a recursion for $\zeta(2n)$ in terms of $\zeta(2n-2k), k=1, \dots n$ - see section \ref{sec:s=n} for further discussion. If the functional equation (\ref{functional}) is used to extend its region of convergence, (\ref{Zsum1a}) becomes

\begin{equation}
\mapleinline{inert}{2d}{zeta(s) =
1/2*Pi^s*Sum(Zeta(1-s+2*k)*(2^(s-2*k-1)-1)/GAMMA(2*k+1)/GAMMA(s-2*k),k
= 1 .. infinity)/(-1+2^(-s))/cos(1/2*Pi*s);}{%
\[
\zeta (s)={\displaystyle \frac {1}{2}} \,{\displaystyle \frac {
\pi ^{s}\, {\displaystyle \sum _{k=1}^{\infty }} \,
{\displaystyle \frac {\zeta (1 - s + 2\,k)\,(2^{s - 2\,k - 1}
 - 1)}{\Gamma (2\,k + 1)\,\Gamma (s - 2\,k)}}  }{( 2^{- s}-1)\,\mathrm{cos}({\displaystyle {\pi \,s/\,2}} 
)}} \hspace*{1cm} \sigma>1
\]
%
}
\end{equation}

which augments similar series appearing in \cite{Sriv}, Sections 4.2 and 4.3, and corresponds to a combination of entries in \cite{Hansen} (Eqs. (54.6.3) and (54.6.4)).

